Embodied-RAG: General Non-parametric Embodied Memory for Retrieval and Generation

There is no limit to how much a robot might explore and learn, but all of that knowledge needs to be searchable and actionable. Within language research, retrieval augmented generation (RAG) has become the workhorse of large-scale non-parametric knowledge; however, existing techniques do not directly transfer to the embodied domain, which is multimodal, where data is highly correlated, and perception requires abstraction. To address these challenges, we introduce Embodied-RAG, a framework that enhances the foundational model of an embodied agent with a non-parametric memory system capable of autonomously constructing hierarchical knowledge for both navigation and language generation. Embodied-RAG handles a full range of spatial and semantic resolutions across diverse environments and query types, whether for a specific object or a holistic description of ambiance. At its core, Embodied-RAG's memory is structured as a semantic forest, storing language descriptions at varying levels of detail. This hierarchical organization allows the system to efficiently generate context-sensitive outputs across different robotic platforms. We demonstrate that Embodied-RAG effectively bridges RAG to the robotics domain, successfully handling over 250 explanation and navigation queries across kilometer-level environments, highlighting its promise as a general-purpose non-parametric system for embodied agents.

==> text/2-problem-formulation.tex <==
% \vspace{-0.5em}

\subsection{Dataset}

The datasets utilized in the Embodied-RAG task are structured as topological graphs. Each node inside the contains an egocentric image, robot coordinates(x,y), a short name, image captions, and caption embeddings.

The dataset is composed of topological graphs designed to capture diverse environmental settings through complementary data collection techniques. Real-world environments were explored using autonomous robots to construct three detailed indoor graphs and one mixed outdoor-indoor graph, capturing realistic navigation scenarios. To model large-scale urban spaces, a comprehensive street-view graph was created using imagery from Google Street View, providing broad and complex spatial data. In parallel, fourteen object topological graphs were generated using the photo-realistic AirSim~\cite{shah2018airsim} simulator, allowing controlled simulation of varied and intricate environments. On average, the topological graphs contain approximately 50 nodes, reflecting moderate complexity in most environments, while the large-scale street-view graph consists of around 3000 nodes, offering extensive spatial coverage for evaluating more complex navigation and retrieval tasks.

\subsection{Embodied-RAG Task}

The Embodied-RAG task is designed to evaluate two fundamental components: retrieval accuracy and generation quality. These components are assessed through two sub-tasks below.

The model processes three query types, explicit(e.g. a retrieve particular object
instance), and implicit (e.g. looking for adequacy, instruction with more pragmatic understanding required), and global quries(e.g. describe the general atmosphere). The global queries that prompt the model to describe the ambiance of a location, explain relationships between environmental elements, or analyze trends within the environment. Unlike the retrieval task, the generation task exclusively produces text-based outputs. The model is expected to deliver coherent and insightful descriptions that align with the provided visual and contextual data (refer to Fig.\ref{fig:figure3_result} top and Fig.\ref{fig:figure2} c-1, as well as Fig.\ref{fig:figure3_result} bottom and Fig.\ref{fig:figure2} c-2).


Examples of these tasks are illustrated in Fig.\ref{fig:figure3_result}, with explicit, implicit, and global queries highlighted in Fig.\ref{fig:figure1}.


\subsection{Evaluation}
Before evaluation, users familiarized themselves with the collected data set to understand the environment by going through the images collected. For each query, three human evaluators give scores simultaneously to the retrieval and generation results. For retrieval tasks, participants chose binary success or failure for the top 1 and top 5 retrieval results, for generation tasks, participants chose based on a likert scale of 1 to 5 to evaluate the quality of the generation.

\subsection{Baselines}
To evaluate our Embodied-RAG approach, we conducted comparative experiments against three baseline methods. The first baseline implements a \textit{Naive RAG} \cite{rag1} adapted for the embodied settings, which retrieves semantically relevant nodes from the topological map and uses them to populate the context window of GPT-4o (with a token limit of 128k), then use it to generate an enhanced response with the results retrieved. The second baseline is GraphRAG\cite{graphrag}, it injects a graph structure into the Naive RAG system. The graph is built by utilizing an LLM to extract entities and relationships from the text, aggregates these text chunks into different communities, and produces a community report to capture global relationships. When retrieval, GraphRAG generates multiple intermediate answers in parallel, one for each chunk, and then sort them based on a helpfulness score and iteratively added into a new context window until the token limit is reached to generate the final answer. The third baseline is LightRAG, the state-of-the-art graphical RAG approach that is much faster in building the knowledge graph, it indexes the graph with a low-level key and a high-level key, and during retrieval it uses this dual-level retrieval method to retrieve the relationships between key entities. 
